Incentivizing Exploration with Selective Data Disclosure

We propose and design recommendation systems that incentivize efficient exploration. Agents arrive sequentially, choose actions and receive rewards, drawn from fixed but unknown action-specific distributions. The recommendation system presents each agent with actions and rewards from a subsequence of past agents, chosen ex ante. Thus, the agents engage in sequential social learning, moderated by these subsequences. We asymptotically attain optimal regret rate for exploration, using a flexible frequentist behavioral model and mitigating rationality and commitment assumptions inherent in prior work. We suggest three components of effective recommendation systems: independent focus groups, group aggregators, and interlaced information structures.

==> abstract-AER.tex <==
We propose and design recommendation systems that incentivize efficient exploration.  Agents arrive sequentially, choose actions and receive rewards, drawn from fixed but unknown action-specific distributions. The recommendation system presents each agent with actions and rewards from a subsequence of past agents, chosen ex ante. Thus, the agents engage in sequential social learning, moderated by these subsequences. We asymptotically attain first-best benchmarks for exploration, using a flexible frequentist behavioral model and mitigating rationality and commitment assumptions inherent in prior work. We suggest three components of effective recommendation systems: independent focus groups, group aggregators, and interlaced information structures.


%We study the design of rating systems that incentivize efficient social learning. Agents arrive sequentially and choose actions, each of which yields a reward drawn from an unknown distribution. A policy maps the rewards of previously-chosen actions to messages for arriving agents. The \emph{regret} of a policy is the difference, over all rounds, between the expected reward of the best action and the reward induced by the policy.  Prior work proposes policies that recommend a single action to each agent, obtaining optimal regret under standard rationality assumptions. We instead assume a frequentist behavioral model and, accordingly, restrict attention to \emph{disclosure policies} that use messages consisting of the actions and rewards from a subsequence of past agents, chosen ex ante. We design a policy with optimal regret in the worst case over reward distributions. Our research suggests three components of effective policies: independent focus groups, group aggregators, and interlaced information structures.


%We study the design of rating systems that incentivize efficient social learning. Agents arrive sequentially and choose actions, each of which yields a positive reward with an unknown probability. A policy maps the rewards of previously-chosen actions to messages for arriving agents. Prior work proposes policies that recommend a single action to each user, obtaining optimal performance under standard rationality assumptions.
%We study disclosure policies that use messages consisting of the actions and rewards from a subsequence of past agents. Each subsequence is chosen ex ante. We posit a flexible model of frequentist agent response, which we argue is plausible for this class of policies. We measure the success of a policy by its \emph{regret}, i.e., the difference, over all rounds, between the expected reward of the best action and the reward induced by the policy.
%We design three policies with regret sublinear in the number of agents $T$.  The first obtains regret $\tilde{O}(T^{2/3})$ by dividing a sublinear number of agents into constant-sized focus groups, whose histories are then revealed to all future agents.  The second improves upon this regret by introducing group aggregators that observe disjoint subsets of focus group histories.  The third obtains regret $\tilde{O}(\sqrt{T})$ by interlacing histories in order to reuse information.  This regret is known to be optimal in the worst case over reward distributions, even absent incentives.

%Our main result is an order-based disclosure policy that obtains regret $\tilde{O}(\sqrt{T})$.  This regret is known to be optimal in the worst case over reward distributions, even absent incentives.  We also exhibit simpler order-based policies with higher, but still sublinear, regret.  The simple policies can be interpreted as dividing a sublinear number of agents into constant-sized focus groups, whose histories are then revealed to future agents.


% Pre-Feb'20 version:
%
%In a social learning setting, there is a set of actions, each of which has a fixed but unknown expected payoff. Agents arrive one by one, each chooses an action with the goal of maximizing the payoff.  A disclosure policy coordinates the choices of the agents by sending messages about the history of past actions. These messages can alter agents' incentives towards \emph{exploration}, taking potentially sub-optimal actions for the sake of learning more about their rewards. The goal of the disclosure policy is to incentivize exploration so as  to maximize social welfare; more specifically, so as to minimize the regret of the action sequence chosen by the agents. Prior work achieves much progress with disclosure policies that merely recommend an action to each user. (Absent agents' incentives, such policy is a multi-armed bandit algorithm.) However, all this work relies heavily on trust and rationality assumptions, standard in economic theory, yet quite problematic in the context of the motivating applications.

%In this paper, we design disclosure policies which incentivize good performance under more plausible behavioral assumptions. Conceptually, we would like to retain the trustworthiness of revealing the full history, while avoiding the herding behavior induced by such disclosure policy (which typically leads to regret linear in the time horizon). We focus on messages, called {\em unbiased subhistories}, consisting of the actions and rewards from a subsequence of past agents, where the subsequence is chosen ahead of time \asedit{according to a predetermined partial order on the rounds.} We posit a flexible model of agent response, which we argue is plausible for this class of \asedit{``order-based"} disclosure policies. Our main result is an \asedit{order-based} disclosure policy that obtains regret $\tilde{O}(\sqrt{T})$, where $T$ is the time horizon.  We also exhibit simpler \asedit{order-based} policies with higher, but still sublinear, regret.  These policies can be interpreted as dividing a sublinear number of agents into constant-sized focus groups, whose histories are then fed to future agents.

% Newer version from Nicole:
%
%We study the design of rating systems that induce optimal learning among frequentist agents.  Agents arrive sequentially and are presented with a set of possible actions, each of which yields a positive reward with an unknown probability.  A disclosure policy sends messages about the rewards of previously-chosen actions to arriving agents.  Agents are frequentists, and so choose actions which (approximately) maximize the empirical mean reward based on their received message.  We study a particular class of disclosure policies that use messages, called unbiased subhistories, consisting of the actions and rewards from a subsequence of past agents, where the subsequence is chosen ahead of time \asedit{according to a predetermined partial order on the rounds.} We posit a flexible model of frequentist agent response, which we argue is plausible for this class of \asedit{``order-based"} disclosure policies. We measure the success of a policy by its induced regret, i.e., the difference, over $T$ rounds, between the expected reward of the best action and the reward induced by the policy.  A disclosure policy that reveals full history in each round risks inducing herding behavior among the agents and thus has regret linear in the number of rounds.  Our main result is an order-based disclosure policy that obtains regret $\tilde{O}(\sqrt{T})$.  This regret is known to be optimal in the worst case over reward distributions, even absent incentives.  We also exhibit simpler order-based policies with higher, but still sublinear, regret.  These policies can be interpreted as dividing a sublinear number of agents into constant-sized focus groups, whose histories are then revealed to future agents.}


==> related-work-detailed.tex <==
%\nidelete{\subsection{Incentivized exploration}}
%\label{sec:related-BIC}

%Let us compare our results and modeling assumptions to those in prior work on incentivized exploration via information asymmetry. Under the strong assumptions inherent in \citet{Kremer-JPE14} and the subsequent work, messaging policies can w.l.o.g. be reduced to multi-armed bandit algorithms which recommend an action to each agent and satisfy  Bayesian incentive-compatibility (\emph{BIC}). Hence, we will refer to this work as the \emph{\OldProblem}.

OBSOLETE SINCE JAN'22

\subsection{BIC Incentivized Exploration}
\label{sec:related-BicIE}

\nimargincomment{I'd like to rename this section Discussion and include the discussion from the model section here instead of in the model section.  This is also a bit repetitive with that and will allow us to tighten the writting.}

\xhdr{Trust and rationality.}
We argue that our trust and rationality assumptions are substantially weaker compared to those in \OldProblem. Several issues are in play:


\vspace{2mm}
\emph{(i) Whether agents understand the announced policy.}
We only need an agent to understand that she is given some \asedit{subhistory which is unbiased and transitive}. It does not matter to the agent what subset of arrivals is covered by this subhistory, and how it is related to the other agents' subsets. This is arguably quite comprehensible, compared to a full-blown specification of a bandit algorithm in \OldProblem.

\vspace{2mm}
\emph{(ii) Whether agents trust the principal to implement the stated policy.}
A third party can, at least in principle, collect rewards and subhistories from multiple agents and audit them for consistency. \asedit{Such audits can be quite powerful: \eg one could take random pairs of agents $t,t'$ which are supposed to satisfy
    $t \in  S_{t'}$ and $S_t\subset  S_{t'}$ ,
and check if this is indeed the case, if the rewards from agents in $S_t$ are reported consistently, and if the reward from agent $t$ is propagated faithfully.
% (\eg, check that arms' average rewards are within the statistical deviations),
The possibility of such audits would} incentivize the principal not to manipulate the policy.

In contrast, bandit algorithms do not readily admit ``external" sanity checks, and are extremely difficult to audit. \asedit{One reason is that} the production code is often intertwined with many other pieces of the system, some of which may change over time or be legitimately non-public.

Moreover, debugging a bandit algorithm tends to be very intricate in realistic applications \citep{DS-arxiv}, so the implementation may deviate from the stated algorithm even if the principal intends otherwise. Faithfully revealing a subhistory is arguably trivial in comparison.


%\emph{(iii) Whether agents trust the principal to implement the stated policy without bugs.} Faithfully revealing a subhistory is arguably easy, whereas debugging a bandit algorithm tends to be very intricate in applications \citep{DS-arxiv}.

\vspace{2mm}
\emph{(iii) Whether agents react as specified.}
%\asedit{As discussed in the Introduction,
Agents in our model can treat the revealed subhistory as (just) a set of data-points, can exhibit a substantial amount of optimism or pessimism, and are not subject to the informational or cognitive load of Bayesian updates.  On the other hand, agents in \OldProblem either need to trust the BIC property or to verify it. The former is arguably a lot to take on faith, and the latter typically requires a sophisticated Bayesian reasoning.
%Whereas incentive-compatibility of a recommendation policy is a lot to take on faith, and  verifying it typically requires a sophisticated Bayesian reasoning.
Moreover, agents may be irrationally averse to recommendations without any supporting information, or to the possibility of being singled out for exploration.



%\subsection{Discussion: machine learning aspects}

%Let us compare the regret rates in prior work on \OldProblem against ours.

\nimargincomment{I believe all this now in related work (where I think it belongs); double check.}
\nidelete{\xhdr{Regret rates.}
\asedit{Let us comment on regret rates in prior work on \OldProblem.}
\citet{ICexploration-ec15} achieve the optimal regret rate \eqref{eq:model-OptRegret} for bandit algorithms without incentives, for a constant number of actions $K$. Their result involves a multiplicative ``constant" that can get arbitrarily large depending on the Bayesian prior. Our result achieves a similar regret rate and similarly depends on a parameter in our choice model.

Prior work either assumes $K=2$ actions \cite[\eg][]{Kremer-JPE14,Che-13,Bimpikis-exploration-ms17,Bahar-ec16}, or targets the case of constant $K$ \citep[\eg][]{ICexploration-ec15,ICexplorationGames-ec16}.
The regret bounds in the latter work, as well as ours, scale exponentially in $K$.
In comparison, bandit algorithms without incentives achieve regret rates that scale as $\sqrt{K}$.

\asedit{In the work subsequent to ours,} \citet{Selke-PoIE-ec21} achieve $\poly(K)$ regret scaling, albeit only when the Bayesian prior is independent across arms and only for Bayesian regret (\ie regret in expectation over the Bayesian prior).
}

\nimargincomment{also in related work i think}
\nidelete{
\subsection{Full disclosure and herding}
\label{sec:related-full}

The full-disclosure policy in \OldProblem reduces to the ``greedy" bandit algorithm which exploits in each round. Its herding effects are most lucidly summarized by focusing on the case of two arms. Then, if arm $1$ is preferable according to the prior, the algorithm never tries arm $2$ with probability at least $\mu^0_1-\mu^0_2$, where $\mu^0_a$ is the prior mean reward of arm $a\in \{1,2\}$. This result holds for an arbitrary priors on rewards, possibly correlated across arms. It implies very high regret (linear in $T$, the number of agents) under additional assumptions, \eg for independent priors with full support. Similar results hold for a frequentist version, where each agent chooses an arm with the highest empirical mean.%
\footnote{For example, consider the case of two arms with Bernoulli rewards, with means $\mu_1>\mu_2$. Assume a ``warm start" such that each arm is tried $N_0$ times, $N_0<(\mu_1-\mu_2)^{-2}$. Then arm $2$ is never chosen with probability at least an absolute constant times $\mu_1-\mu_2$. This holds under a mild assumption on $\mu_1,\mu_2$, \eg
    $\nicefrac18 + \mu_1-\mu_2 \leq \mu_2 <\mu_1 \leq \nicefrac78$.}
These results can be found in
    \citep[Chapter 11.2 in][]{slivkins-MABbook}.
Various weaker versions have been ``folklore" for decades.
}

\nimargincomment{not all in related work, but not necessary imo}
\nidelete{
\subsection{Social learning}
\label{sec:related-social}

A large literature on \emph{social learning} studies agents that learn over time in a shared environment, with no principal to coordinate them. A prominent topic is the  presence or absence of herding phenomena.  Models vary across several dimensions, to wit:
how an agent acquires new information;
which information is transmitted to others;
what is the structure / properties of the communication network;
whether agents are long-lived or only act once;
whether they optimize rewards (via Bayesian rationality or frequentist behavior), or merely follow a rule-of-thumb.
%While our work can be interpreted as coordinating social learning, all prior work studies models of social learning that are very different from ours.
Below we discuss three lines of work in social learning that are most relevant, and point our the major differences compared to our model.

First, ``sequential social learning" posits that agents observe private signals, but only the chosen actions of neighbors are observable in the future; see \cite{Golub-survey16} for a survey.
The early work focuses on \asdelete{sequential learning over} a complete communication network, starting from \cite{Banerjee-qje92,Welch92,Bikhchandani-jpe92}, with a very general result in \citet{SmithSorensen-econometrica00}. Further work considers the impact of the network topology \asdelete{on sequential learning}.  In particular, \cite{acemoglu2011bayesian} and \cite{lobel2015information} show that in a perfect Bayesian equilibrium, learning happens asymptotically if neighborhoods are sufficiently expansive or independent, features echoed in our own constructions.
%Sparse network topologies are studied in \citet{BogachanKariv-geb04,Banerjee-geb04,Acemoglu-te14}
To contrast these models with ours, we emphasize that the social planner only needs to choose the best action given the previous agents' signals, \ie only needs to \emph{exploit}, whereas in our model it also needs to \emph{explore}. Also, herding occurs due to restricted information flow between the agents, whereas in our model it happens even with full disclosure.

Another line of work, starting from \citet{DeGroot74}, posits that agents use ``naive", mechanical rules-of-thumb, \eg form beliefs based on naive averaging of observations.%
\footnote{Our frequentist agents may behave similarly, albeit  with more justification (because the subhistories they observe are unbiased and transitive). The original paper of \citet{DeGroot74} and much subsequent work study agents that act repeatedly, updating their beliefs over rounds.} In particular, even naive agents learn asymptotically so long as the network is not too imbalanced \citep[\eg][]{golub2010naive}.
\cite{chandrasekhar2020testing}
show experimentally that such a behavioral model is a good predictor of human behavior in some scenarios.
\cite{dasaratha2019experiment} show similar results for sequential social learning.  Theoretically, \cite{dasaratha2020learning} use this model of naivety to study the question of how to design the social network in a sequential learning model so as to induce optimal learning rates. They observe that silo structures akin to our two-level policy improve learning rates.

%Another line of work on observational social learning studies a model in which agents act repeatedly, updating beliefs over rounds.  There are two prominent models of behavior here: Bayesian rationality and naivety or DeGroot dynamics \citep{DeGroot74}, in which agents form beliefs based on naive averaging of observations (similar to our frequentist agents).  Prior work shows that even naive agents learn asymptotically so long as the network is not too imbalanced \citep[\eg][]{golub2010naive}. \cite{chandrasekhar2020testing} show experimentally that such a behavioral model in fact better predicts agent behavior in some settings, e.g., in an experiment in Indian villages, naivety better-predicted agent behavior 90\% of the time.  \cite{dasaratha2019experiment} show similar results in the sequential social learning setting.  Theoretically, \cite{dasaratha2020learning} use this model of naivety to study the question of how to design the network to induce optimal learning rates in a sequential learning model.  They observe silo structures akin to our two-level model improve learning rates.

Third, ``strategic experimentation'', starting from \citet{Bolton-econometrica99,Keller-econometrica05}, studies long-lived learning agents that observe both actions and rewards of one another; see \citet{Horner-survey16} for a survey. This is similar to our work in that the social planner also solves a version of multi-armed bandits. The main difference is that the agents are long-lived and engage in a complex repeated game where each player deploys an exploration policy but would prefer to free-ride on exploration by others. There are also important technical differences. Agents exactly optimize their Bayesian-expected utility (using the Markov Perfect Equilibrium as a solution concept), whereas we consider a flexible frequentist model. Also, the social-planner problem is a very \emph{different} bandit problem, with Bayesian prior, time-discounting, ``safe" arm that is completely known, and ``risky" arm that follows a stochastic process.
} 
